She's Got Her Mother's Hair: Unveiling the Origin of Black Hole Magnetic Fields through Stellar to Collapsar Simulations

Relativistic jets from a Kerr black hole (BH) following the core collapse of a massive star ("collapsar") is a leading model for gamma-ray bursts (GRBs). However, the two key ingredients for a Blandford-Znajek powered jet $-$ rapid rotation and a strong magnetic field $-$ seem mutually exclusive. Strong fields in the progenitor star's core transport angular momentum outwards more quickly, slowing down the core before collapse. Through innovative multidisciplinary modeling, we first use MESA stellar evolution models followed to core collapse, to explicitly show that the small length-scale of the instabilities $-$ likely responsible for angular momentum transport in the core (e.g., Tayler-Spruit) $ - $ results in a low net magnetic flux fed to the BH horizon, far too small to power GRB jets. Instead, we propose a novel scenario in which collapsar BHs acquire their magnetic "hair" from their progenitor proto-neutron star (PNS), which is likely highly magnetized from an internal dynamo. We evaluate the conditions for the BH accretion disk to pin the PNS magnetosphere to its horizon immediately after the collapse. Our results show that the PNS spin-down energy released before collapse matches the kinetic energy of Type Ic-BL supernovae, while the nascent BH's spin and magnetic flux produce jets consistent with observed GRB characteristics. We map our MESA models to 3D general-relativistic magnetohydrodynamic simulations and confirm that accretion disks confine the strong magnetic flux initiated near a rotating BH, enabling the launch of successful GRB jets, whereas a slower-spinning BH or one without a disk fails to do so.

==> MESA_input/re <==
#!/bin/bash

# shopt -u expand_aliases

photo_directory=photos

function most_recent_photo {
    ls -tp "$photo_directory" | grep -v / | head -1
}

if [ $# -eq 0 ]
then
    photo=$(most_recent_photo)
else
    photo=$1
fi

if [ -z "$photo" ] || ! [ -f "$photo_directory/$photo" ]
then
    echo "specified photo ($photo) does not exist"
    exit 1
fi

echo "restart from $photo"
if ! cp "$photo_directory/$photo" restart_photo
then
    echo "failed to copy photo ($photo)"
    exit 1
fi

{
    date "+DATE: %Y-%m-%d%nTIME: %H:%M:%S"
    ./star
    date "+DATE: %Y-%m-%d%nTIME: %H:%M:%S"
} 2>&1 | tee output_restart.txt ;


# try to find last png
png=$(find  -path "./png/single*.png" -printf "%T@ %P\n" | sort -n | tail -1 | awk '{print $2}');
tail -n 50 output_restart.txt | mail -A $png -a "From:simulations@arizona.edu" -s "ua_w done" mrenzo@arizona.edu


==> MESA_input/rn <==
#!/bin/bash

{
    rm -f restart_photo

    date "+DATE: %Y-%m-%d%nTIME: %H:%M:%S"
    ./star
    date "+DATE: %Y-%m-%d%nTIME: %H:%M:%S"
} 2>&1 | tee output.txt ;

# try to find last png
png=$(find  -path "./png/single*.png" -printf "%T@ %P\n" | sort -n | tail -1 | awk '{print $2}') ;
tail -n 50 output.txt | mail -A $png -a "From:simulations@arizona.edu" -s "ua_w done" mrenzo@arizona.edu


==> Referee.tex <==
We thank the referee for the positive review. Below we address the referee's concerns.

This is a carefully-written and well-presented paper mapping GRB progenitor star MESA models into 3D GRMHD collapsar simulations after black-hole formation. I find the paper very well-prepared and it demonstrates important results justifying publication in ApJ Letters. My main point of criticism is that I do not find the title and presentation of the paper as an 'end-to-end simulation' appropriate as the authors do not simulate the crucial phase of the proto-neutron-star evolution possibly accompanied by an MHD-powered supernova explosion. I describe this and some other minor points that I would like the authors to address before publication in more detail below:

- As mention above, I do think the presentation of the paper as end-to-end simulation is misleading to readers that may not be intricately aware of the different phases occuring between stellar evolution models at the beginning and black-hole powered collapsar jets at the end. While the authors carefully argue their choices for the setup of the black hole + disk system for the collapsar simulations, they do not perform simulations of the PNS evolution and potential core-collapse supernova during this phase and I don't think that is clear from the way the paper is written. It would be better if the authors could clarify this and also mention caveats in the discussion.

-> We agree with the referee that this is not a fully self-consistent, end-to-end simulation without modeling the PNS phase. In response, we have revised the title and instead highlighted the novelty of our multidisciplinary approach in linking stellar evolution to post-explosion dynamics. Additionally, we have clarified that the simulations do not include the CCSN and PNS phases, as suggested by the referee.

- The authors state in Sec. 3.1 that a centrifugally-supported disk is likely already present around the PNS. Can they argue this in more detail or back it up with a reference? Is this actually seen in CCSN simulations of these systems? This matters quite a bit for the setup chosen for the GRMHD black hole simulations the authors set up later and would seem important to understand better to judge how realistic the chosen setups are.

-> The early disk formation is demonstrated in Figure 2(a) and discussed in the text. We reach the same conclusions by performing the same calculation based on models by Woosley & Heger (2006). The excess angular momentum during the PNS phase, which leads to a disk formation, was also discussed by Dessart et al. 2008. We revised the text and highlighted the relevant parts discussing this aspect.

- In the introduction I think citing Mösta 2014 (ApJL) when mentioning jets powered from a NS could be a good addition to clarify that it's not always easy to get a GRB jet from PNS outflows in realistic CCSN simulations.

-> We added a reference to Mösta 2014 in the introduction.

==> scripts/matplotlibrc <==
#### MATPLOTLIBRC FORMAT

# author: Mathieu Renzo

## This is a sample matplotlib configuration file - you can find a copy
## of it on your system in
## site-packages/matplotlib/mpl-data/matplotlibrc.  If you edit it
## there, please note that it will be overwritten in your next install.
## If you want to keep a permanent local copy that will not be
## overwritten, place it in the following location:
## unix/linux:
##      $HOME/.config/matplotlib/matplotlibrc or
##      $XDG_CONFIG_HOME/matplotlib/matplotlibrc (if $XDG_CONFIG_HOME is set)
## other platforms:
##      $HOME/.matplotlib/matplotlibrc
##
## See http://matplotlib.org/users/customizing.html#the-matplotlibrc-file for
## more details on the paths which are checked for the configuration file.
##
## This file is best viewed in a editor which supports python mode
## syntax highlighting. Blank lines, or lines starting with a comment
## symbol, are ignored, as are trailing comments.  Other lines must
## have the format
##     key : val ## optional comment
##
## Colors: for the color values below, you can either use - a
## matplotlib color string, such as r, k, or b - an rgb tuple, such as
## (1.0, 0.5, 0.0) - a hex string, such as ff00ff - a scalar
## grayscale intensity such as 0.75 - a legal html color name, e.g., red,
## blue, darkslategray

##### CONFIGURATION BEGINS HERE

## The default backend. If you omit this parameter, the first
## working backend from the following list is used:
## MacOSX Qt5Agg Qt4Agg Gtk3Agg TkAgg WxAgg Agg
##
## Other choices include:
## Qt5Cairo Qt4Cairo GTK3Cairo TkCairo WxCairo Cairo Wx PS PDF SVG Template.
##
## You can also deploy your own backend outside of matplotlib by
## referring to the module name (which must be in the PYTHONPATH) as
## 'module://my_backend'.
#backend      : Agg

## Note that this can be overridden by the environment variable
## QT_API used by Enthought Tool Suite (ETS); valid values are
## "pyqt" and "pyside".  The "pyqt" setting has the side effect of
## forcing the use of Version 2 API for QString and QVariant.

## The port to use for the web server in the WebAgg backend.
#webagg.port : 8988

## The address on which the WebAgg web server should be reachable
#webagg.address : 127.0.0.1

## If webagg.port is unavailable, a number of other random ports will
## be tried until one that is available is found.
#webagg.port_retries : 50

## When True, open the webbrowser to the plot that is shown
#webagg.open_in_browser : True

## if you are running pyplot inside a GUI and your backend choice
## conflicts, we will automatically try to find a compatible one for
## you if backend_fallback is True
#backend_fallback: True

#interactive  : False
#toolbar      : toolbar2   ## None | toolbar2  ("classic" is deprecated)
#timezone     : UTC        ## a pytz timezone string, e.g., US/Central or Europe/Paris

## Where your matplotlib data lives if you installed to a non-default
## location.  This is where the matplotlib fonts, bitmaps, etc reside
#datapath : /home/jdhunter/mpldata


#### LINES
## See http://matplotlib.org/api/artist_api.html#module-matplotlib.lines for more
## information on line properties.
lines.linewidth   : 3     ## line width in points
#lines.linestyle   : -       ## solid line
#lines.color       : C0      ## has no affect on plot(); see axes.prop_cycle
#lines.marker      : None    ## the default marker
#lines.markerfacecolor  : auto    ## the default markerfacecolor
#lines.markeredgecolor  : auto    ## the default markeredgecolor
lines.markeredgewidth  : 2.0     ## the line width around the marker symbol
#lines.markersize  : 6            ## markersize, in points
#lines.dash_joinstyle : round        ## miter|round|bevel
#lines.dash_capstyle : butt          ## butt|round|projecting
#lines.solid_joinstyle : round       ## miter|round|bevel
#lines.solid_capstyle : projecting   ## butt|round|projecting
#lines.antialiased : True         ## render lines in antialiased (no jaggies)

## The three standard dash patterns.  These are scaled by the linewidth.
#lines.dashed_pattern : 3.7, 1.6
#lines.dashdot_pattern : 6.4, 1.6, 1, 1.6
#lines.dotted_pattern : 1, 1.65
#lines.scale_dashes : True

#markers.fillstyle: full ## full|left|right|bottom|top|none

#### PATCHES
## Patches are graphical objects that fill 2D space, like polygons or
## circles.  See
## http://matplotlib.org/api/artist_api.html#module-matplotlib.patches
## information on patch properties
#patch.linewidth        : 1        ## edge width in points.
#patch.facecolor        : C0
#patch.edgecolor        : black   ## if forced, or patch is not filled
#patch.force_edgecolor  : False   ## True to always use edgecolor
#patch.antialiased      : True    ## render patches in antialiased (no jaggies)

#### HATCHES
#hatch.color     : black
#hatch.linewidth : 1.0

#### Boxplot
#boxplot.notch       : False
#boxplot.vertical    : True
#boxplot.whiskers    : 1.5
#boxplot.bootstrap   : None
#boxplot.patchartist : False
#boxplot.showmeans   : False
#boxplot.showcaps    : True
#boxplot.showbox     : True
#boxplot.showfliers  : True
#boxplot.meanline    : False

#boxplot.flierprops.color           : black
#boxplot.flierprops.marker          : o
#boxplot.flierprops.markerfacecolor : none
#boxplot.flierprops.markeredgecolor : black
#boxplot.flierprops.markeredgewidth : 1.0
#boxplot.flierprops.markersize      : 6
#boxplot.flierprops.linestyle       : none
#boxplot.flierprops.linewidth       : 1.0

#boxplot.boxprops.color     : black
#boxplot.boxprops.linewidth : 1.0
#boxplot.boxprops.linestyle : -

#boxplot.whiskerprops.color     : black
#boxplot.whiskerprops.linewidth : 1.0
#boxplot.whiskerprops.linestyle : -

#boxplot.capprops.color     : black
#boxplot.capprops.linewidth : 1.0
#boxplot.capprops.linestyle : -

#boxplot.medianprops.color     : C1
#boxplot.medianprops.linewidth : 1.0
#boxplot.medianprops.linestyle : -

#boxplot.meanprops.color           : C2
#boxplot.meanprops.marker          : ^
#boxplot.meanprops.markerfacecolor : C2
#boxplot.meanprops.markeredgecolor : C2
#boxplot.meanprops.markersize      :  6
#boxplot.meanprops.linestyle       : --
#boxplot.meanprops.linewidth       : 1.0


#### FONT

## font properties used by text.Text.  See
## http://matplotlib.org/api/font_manager_api.html for more
## information on font properties.  The 6 font properties used for font
## matching are given below with their default values.
##
## The font.family property has five values: 'serif' (e.g., Times),
## 'sans-serif' (e.g., Helvetica), 'cursive' (e.g., Zapf-Chancery),
## 'fantasy' (e.g., Western), and 'monospace' (e.g., Courier).  Each of
## these font families has a default list of font names in decreasing
## order of priority associated with them.  When text.usetex is False,
## font.family may also be one or more concrete font names.
##
## The font.style property has three values: normal (or roman), italic
## or oblique.  The oblique style will be used for italic, if it is not
## present.
##
## The font.variant property has two values: normal or small-caps.  For
## TrueType fonts, which are scalable fonts, small-caps is equivalent
## to using a font size of 'smaller', or about 83%% of the current font
## size.
##
## The font.weight property has effectively 13 values: normal, bold,
## bolder, lighter, 100, 200, 300, ..., 900.  Normal is the same as
## 400, and bold is 700.  bolder and lighter are relative values with
## respect to the current weight.
##
## The font.stretch property has 11 values: ultra-condensed,
## extra-condensed, condensed, semi-condensed, normal, semi-expanded,
## expanded, extra-expanded, ultra-expanded, wider, and narrower.  This
## property is not currently implemented.
##
## The font.size property is the default font size for text, given in pts.
## 10 pt is the standard value.

font.family         : serif
#font.style          : normal
#font.variant        : normal
# font.weight          : normal
#font.stretch        : normal
## note that font.size controls default text sizes.  To configure
## special text sizes tick labels, axes, labels, title, etc, see the rc
## settings for axes and ticks. Special text sizes can be defined
## relative to font.size, using the following values: xx-small, x-small,
## small, medium, large, x-large, xx-large, larger, or smaller
#font.size           : 10.0
font.serif          : cmr10 # DejaVu Serif, Bitstream Vera Serif, Computer Modern Roman, New Century Schoolbook, Century Schoolbook L, Utopia, ITC Bookman, Bookman, Nimbus Roman No9 L, Times New Roman, Times, Palatino, Charter, serif
font.sans-serif     : cmr10 # DejaVu Sans, Bitstream Vera Sans, Computer Modern Sans Serif, Lucida Grande, Verdana, Geneva, Lucid, Arial, Helvetica, Avant Garde, sans-serif
#font.cursive        : Apple Chancery, Textile, Zapf Chancery, Sand, Script MT, Felipa, cursive
#font.fantasy        : Comic Sans MS, Chicago, Charcoal, ImpactWestern, Humor Sans, xkcd, fantasy
#font.monospace      : DejaVu Sans Mono, Bitstream Vera Sans Mono, Computer Modern Typewriter, Andale Mono, Nimbus Mono L, Courier New, Courier, Fixed, Terminal, monospace

#### TEXT
## text properties used by text.Text.  See
## http://matplotlib.org/api/artist_api.html#module-matplotlib.text for more
## information on text properties
#text.color          : black

#### LaTeX customizations. See http://wiki.scipy.org/Cookbook/Matplotlib/UsingTex
text.usetex         : False    ## use latex for all text handling. The following fonts
                              ## are supported through the usual rc parameter settings:
                              ## new century schoolbook, bookman, times, palatino,
                              ## zapf chancery, charter, serif, sans-serif, helvetica,
                              ## avant garde, courier, monospace, computer modern roman,
                              ## computer modern sans serif, computer modern typewriter
                              ## If another font is desired which can loaded using the
                              ## LaTeX \usepackage command, please inquire at the
                              ## matplotlib mailing list
#text.latex.preamble :      ## IMPROPER USE OF THIS FEATURE WILL LEAD TO LATEX FAILURES
                            ## AND IS THEREFORE UNSUPPORTED. PLEASE DO NOT ASK FOR HELP
                            ## IF THIS FEATURE DOES NOT DO WHAT YOU EXPECT IT TO.
                            ## text.latex.preamble is a single line of LaTeX code that
                            ## will be passed on to the LaTeX system. It may contain
                            ## any code that is valid for the LaTeX "preamble", i.e.
                            ## between the "\documentclass" and "\begin{document}"
                            ## statements.
                            ## Note that it has to be put on a single line, which may
                            ## become quite long.
                            ## The following packages are always loaded with usetex, so
                            ## beware of package collisions: color, geometry, graphicx,
                            ## type1cm, textcomp.
                            ## Adobe Postscript (PSSNFS) font packages may also be
                            ## loaded, depending on your font settings.
#text.latex.preview : False

#text.hinting : auto   ## May be one of the following:
                       ##   none: Perform no hinting
                       ##   auto: Use FreeType's autohinter
                       ##   native: Use the hinting information in the
                       #              font file, if available, and if your
                       #              FreeType library supports it
                       ##   either: Use the native hinting information,
                       #              or the autohinter if none is available.
                       ## For backward compatibility, this value may also be
                       ## True === 'auto' or False === 'none'.
#text.hinting_factor : 8 ## Specifies the amount of softness for hinting in the
                         ## horizontal direction.  A value of 1 will hint to full
                         ## pixels.  A value of 2 will hint to half pixels etc.
#text.antialiased : True ## If True (default), the text will be antialiased.
                         ## This only affects the Agg backend.

## The following settings allow you to select the fonts in math mode.
## They map from a TeX font name to a fontconfig font pattern.
## These settings are only used if mathtext.fontset is 'custom'.
## Note that this "custom" mode is unsupported and may go away in the
## future.
#mathtext.cal : cursive
#mathtext.rm  : sans
#mathtext.tt  : monospace
#mathtext.it  : sans:italic
#mathtext.bf  : sans:bold
#mathtext.sf  : sans
mathtext.fontset : cm #dejavusans ## Should be 'dejavusans' (default),
                               ## 'dejavuserif', 'cm' (Computer Modern), 'stix',
                               ## 'stixsans' or 'custom'
# mathtext.fallback_to_cm : True  ## When True, use symbols from the Computer Modern
                                 ## fonts when a symbol can not be found in one of
                                 ## the custom math fonts.
mathtext.default : regular  ## The default font to use for math.
                       ## Can be any of the LaTeX font names, including
                       ## the special name "regular" for the same font
                       ## used in regular text.

#### AXES
## default face and edge color, default tick sizes,
## default fontsizes for ticklabels, and so on.  See
## http://matplotlib.org/api/axes_api.html#module-matplotlib.axes
axes.facecolor      : white   ## axes background color
#axes.edgecolor      : black   ## axes edge color
axes.linewidth       : 2     ## edge linewidth
#axes.grid           : False   ## display grid or not
#axes.grid.axis      : both    ## which axis the grid should apply to
#axes.grid.which     : major   ## gridlines at major, minor or both ticks
#axes.titlesize      : large   ## fontsize of the axes title
#axes.titleweight    : normal  ## font weight of title
#axes.titlepad       : 6.0     ## pad between axes and title in points
axes.labelsize       : 30  ## fontsize of the x any y labels
axes.labelpad        : 2	        ## space between label and axis
#axes.labelweight    : normal  ## weight of the x and y labels
#axes.labelcolor     : black
#axes.axisbelow      : line    ## draw axis gridlines and ticks below
                               ## patches (True); above patches but below
                               ## lines ('line'); or above all (False)
#axes.formatter.limits : -7, 7 ## use scientific notation if log10
                               ## of the axis range is smaller than the
                               ## first or larger than the second
#axes.formatter.use_locale : False ## When True, format tick labels
                                   ## according to the user's locale.
                                   ## For example, use ',' as a decimal
                                   ## separator in the fr_FR locale.
axes.formatter.use_mathtext : True ## When True, use mathtext for scientific
                                     ## notation.
#axes.formatter.min_exponent: 0 ## minimum exponent to format in scientific notation
#axes.formatter.useoffset      : True    ## If True, the tick label formatter
                                         ## will default to labeling ticks relative
                                         ## to an offset when the data range is
                                         ## small compared to the minimum absolute
                                         ## value of the data.
#axes.formatter.offset_threshold : 4     ## When useoffset is True, the offset
                                         ## will be used when it can remove
                                         ## at least this number of significant
                                         ## digits from tick labels.
#axes.spines.left   : True   ## display axis spines
#axes.spines.bottom : True
#axes.spines.top    : True
#axes.spines.right  : True
axes.unicode_minus  : False    ## use unicode for the minus symbol
                               ## rather than hyphen.  See
                               ## http://en.wikipedia.org/wiki/Plus_and_minus_signs#Character_codes
#axes.prop_cycle    : cycler('color', ['1f77b4', 'ff7f0e', '2ca02c', 'd62728', '9467bd', '8c564b', 'e377c2', '7f7f7f', 'bcbd22', '17becf'])
                      ## color cycle for plot lines  as list of string
                      ## colorspecs: single letter, long name, or web-style hex
					  ## Note the use of string escapes here ('1f77b4', instead of 1f77b4)
                      ## as opposed to the rest of this file.
#axes.autolimit_mode : data ## How to scale axes limits to the data.
                            ## Use "data" to use data limits, plus some margin
                            ## Use "round_number" move to the nearest "round" number
#axes.xmargin        : .05  ## x margin.  See `axes.Axes.margins`
#axes.ymargin        : .05  ## y margin See `axes.Axes.margins`
#polaraxes.grid      : True    ## display grid on polar axes
#axes3d.grid         : True    ## display grid on 3d axes

#### DATES
## These control the default format strings used in AutoDateFormatter.
## Any valid format datetime format string can be used (see the python
## `datetime` for details).  For example using '%%x' will use the locale date representation
## '%%X' will use the locale time representation and '%%c' will use the full locale datetime
## representation.
## These values map to the scales:
##     {'year': 365, 'month': 30, 'day': 1, 'hour': 1/24, 'minute': 1 / (24 * 60)}

#date.autoformatter.year     : %Y
#date.autoformatter.month    : %Y-%m
#date.autoformatter.day      : %Y-%m-%d
#date.autoformatter.hour     : %m-%d %H
#date.autoformatter.minute   : %d %H:%M
#date.autoformatter.second   : %H:%M:%S
#date.autoformatter.microsecond   : %M:%S.%f

#### TICKS
## see http://matplotlib.org/api/axis_api.html#matplotlib.axis.Tick
xtick.top             : True  ## draw ticks on the top side
#xtick.bottom         : True   ## draw ticks on the bottom side
#xtick.labeltop       : False  ## draw label on the top
#xtick.labelbottom    : True   ## draw label on the bottom
xtick.major.size      : 12    ## major tick size in points
xtick.minor.size      : 6      ## minor tick size in points
xtick.major.width     : 2    ## major tick width in points
xtick.minor.width     : 2    ## minor tick width in points
xtick.major.pad       : 12    ## distance to major tick label in points
#xtick.minor.pad      : 3.4    ## distance to the minor tick label in points
#xtick.color          : black  ## color of the tick labels
xtick.labelsize       : 30 ## fontsize of the tick labels
xtick.direction       : in    ## direction: in, out, or inout
xtick.minor.visible   : True  ## visibility of minor ticks on x-axis
#xtick.major.top      : True   ## draw x axis top major ticks
#xtick.major.bottom   : True   ## draw x axis bottom major ticks
#xtick.minor.top      : True   ## draw x axis top minor ticks
#xtick.minor.bottom   : True   ## draw x axis bottom minor ticks
#xtick.alignment      : center ## alignment of xticks

#ytick.left           : True   ## draw ticks on the left side
ytick.right           : True  ## draw ticks on the right side
#ytick.labelleft      : True   ## draw tick labels on the left side
#ytick.labelright     : False  ## draw tick labels on the right side
ytick.major.size      : 12    ## major tick size in points
ytick.minor.size      : 6     ## minor tick size in points
ytick.major.width     : 2    ## major tick width in points
ytick.minor.width     : 2    ## minor tick width in points
ytick.major.pad       : 12    ## distance to major tick label in points
#ytick.minor.pad      : 3.4    ## distance to the minor tick label in points
#ytick.color          : black  ## color of the tick labels
ytick.labelsize       : 30 ## fontsize of the tick labels
ytick.direction       : in    ## direction: in, out, or inout
ytick.minor.visible  : True  ## visibility of minor ticks on y-axis
#ytick.major.left     : True   ## draw y axis left major ticks
#ytick.major.right    : True   ## draw y axis right major ticks
#ytick.minor.left     : True   ## draw y axis left minor ticks
#ytick.minor.right    : True   ## draw y axis right minor ticks
#ytick.alignment      : center_baseline ## alignment of yticks

#### GRIDS
#grid.color       :   b0b0b0    ## grid color
#grid.linestyle   :   -         ## solid
#grid.linewidth   :   0.8       ## in points
#grid.alpha       :   1.0       ## transparency, between 0.0 and 1.0

#### Legend
#legend.loc           : best
legend.frameon       : False     ## if True, draw the legend on a background patch
#legend.framealpha    : 0.8      ## legend patch transparency
#legend.facecolor     : inherit  ## inherit from axes.facecolor; or color spec
#legend.edgecolor     : 0.8      ## background patch boundary color
#legend.fancybox      : True     ## if True, use a rounded box for the
                                 ## legend background, else a rectangle
#legend.shadow        : False    ## if True, give background a shadow effect
#legend.numpoints     : 1        ## the number of marker points in the legend line
#legend.scatterpoints : 1        ## number of scatter points
#legend.markerscale   : 1.0      ## the relative size of legend markers vs. original
legend.fontsize       : 30
legend.title_fontsize : 30 ## None sets to the same as the default axes.
## Dimensions as fraction of fontsize:
legend.borderpad     : 0.2      ## border whitespace
#legend.labelspacing  : 0.5      ## the vertical space between the legend entries
legend.handlelength  : 1.5      ## the length of the legend lines
legend.handleheight  : 0.4      ## the height of the legend handle
#legend.handletextpad : 0.8      ## the space between the legend line and legend text
#legend.borderaxespad : 0.5      ## the border between the axes and legend edge
legend.columnspacing : 1.6      ## column separation

#### FIGURE
## See http://matplotlib.org/api/figure_api.html#matplotlib.figure.Figure
figure.titlesize : 30     ## size of the figure title (Figure.suptitle())
#figure.titleweight : normal   ## weight of the figure title
figure.figsize   : 8, 8   ## figure size in inches
# figure.dpi       : 100        ## figure dots per inch
figure.facecolor : white      ## figure facecolor
figure.edgecolor : white      ## figure edgecolor
figure.frameon : True         ## enable figure frame
figure.max_open_warning : 10  ## The maximum number of figures to open through
                               ## the pyplot interface before emitting a warning.
                               ## If less than one this feature is disabled.
## The figure subplot parameters.  All dimensions are a fraction of the
#figure.subplot.left    : 0.125  ## the left side of the subplots of the figure
#figure.subplot.right   : 0.9    ## the right side of the subplots of the figure
#figure.subplot.bottom  : 0.11   ## the bottom of the subplots of the figure
#figure.subplot.top     : 0.88   ## the top of the subplots of the figure
#figure.subplot.wspace  : 0.2    ## the amount of width reserved for space between subplots,
                                 ## expressed as a fraction of the average axis width
#figure.subplot.hspace  : 0.2    ## the amount of height reserved for space between subplots,
                                 ## expressed as a fraction of the average axis height

## Figure layout
figure.autolayout : True       ## When True, automatically adjust subplot
                               ## parameters to make the plot fit the figure
                               ## using `tight_layout`
#figure.constrained_layout.use: False ## When True, automatically make plot
                                      ## elements fit on the figure. (Not compatible
                                      ## with `autolayout`, above).
#figure.constrained_layout.h_pad : 0.04167 ## Padding around axes objects. Float representing
#figure.constrained_layout.w_pad : 0.04167 ##  inches. Default is 3./72. inches (3 pts)
#figure.constrained_layout.hspace : 0.02   ## Space between subplot groups. Float representing
#figure.constrained_layout.wspace : 0.02   ##  a fraction of the subplot widths being separated.

#### IMAGES
#image.aspect : equal             ## equal | auto | a number
#image.interpolation  : nearest   ## see help(imshow) for options
image.cmap   : viridis           ## A colormap name, gray etc...
#image.lut    : 256               ## the size of the colormap lookup table
#image.origin : upper             ## lower | upper
#image.resample  : True
#image.composite_image : True     ## When True, all the images on a set of axes are
                                  ## combined into a single composite image before
                                  ## saving a figure as a vector graphics file,
                                  ## such as a PDF.

#### CONTOUR PLOTS
#contour.negative_linestyle : dashed ## string or on-off ink sequence
#contour.corner_mask        : True   ## True | False | legacy

#### ERRORBAR PLOTS
errorbar.capsize : 2             ## length of end cap on error bars in pixels

#### HISTOGRAM PLOTS
#hist.bins : 10                   ## The default number of histogram bins.
                                  ## If Numpy 1.11 or later is
                                  ## installed, may also be `auto`

#### SCATTER PLOTS
#scatter.marker : o               ## The default marker type for scatter plots.
#scatter.edgecolors : face        ## The default edgecolors for scatter plots.

#### Agg rendering
#### Warning: experimental, 2008/10/10
#agg.path.chunksize : 0           ## 0 to disable; values in the range
                                  ## 10000 to 100000 can improve speed slightly
                                  ## and prevent an Agg rendering failure
                                  ## when plotting very large data sets,
                                  ## especially if they are very gappy.
                                  ## It may cause minor artifacts, though.
                                  ## A value of 20000 is probably a good
                                  ## starting point.
#### PATHS
#path.simplify : True   ## When True, simplify paths by removing "invisible"
                        ## points to reduce file size and increase rendering
                        ## speed
#path.simplify_threshold : 0.111111111111  ## The threshold of similarity below which
                                           ## vertices will be removed in the
                                           ## simplification process
#path.snap : True ## When True, rectilinear axis-aligned paths will be snapped to
                  ## the nearest pixel when certain criteria are met.  When False,
                  ## paths will never be snapped.
#path.sketch : None ## May be none, or a 3-tuple of the form (scale, length,
                    ## randomness).
                    ## *scale* is the amplitude of the wiggle
                    ## perpendicular to the line (in pixels).  *length*
                    ## is the length of the wiggle along the line (in
                    ## pixels).  *randomness* is the factor by which
                    ## the length is randomly scaled.
#path.effects : []  ##

#### SAVING FIGURES
## the default savefig params can be different from the display params
## e.g., you may want a higher resolution, or to make the figure
## background white
savefig.dpi         : figure   ## figure dots per inch or 'figure'
savefig.facecolor   : white    ## figure facecolor when saving
savefig.edgecolor   : white    ## figure edgecolor when saving
#savefig.format      : png      ## png, ps, pdf, svg
savefig.bbox        : tight ## 'tight' or 'standard'.
                                ## 'tight' is incompatible with pipe-based animation
                                ## backends but will workd with temporary file based ones:
                                ## e.g. setting animation.writer to ffmpeg will not work,
                                ## use ffmpeg_file instead
#savefig.pad_inches  : 0.1      ## Padding to be used when bbox is set to 'tight'
#savefig.jpeg_quality: 95       ## when a jpeg is saved, the default quality parameter.
#savefig.directory   : ~        ## default directory in savefig dialog box,
                                ## leave empty to always use current working directory
#savefig.transparent : False    ## setting that controls whether figures are saved with a
                                ## transparent background by default
#savefig.orientation : portrait	## Orientation of saved figure

### tk backend params
#tk.window_focus   : False    ## Maintain shell focus for TkAgg

### ps backend params
#ps.papersize      : letter   ## auto, letter, legal, ledger, A0-A10, B0-B10
#ps.useafm         : False    ## use of afm fonts, results in small files
#ps.usedistiller   : False    ## can be: None, ghostscript or xpdf
                                          ## Experimental: may produce smaller files.
                                          ## xpdf intended for production of publication quality files,
                                          ## but requires ghostscript, xpdf and ps2eps
#ps.distiller.res  : 6000      ## dpi
#ps.fonttype       : 3         ## Output Type 3 (Type3) or Type 42 (TrueType)

### pdf backend params
#pdf.compression   : 6   ## integer from 0 to 9
                         ## 0 disables compression (good for debugging)
#pdf.fonttype       : 3         ## Output Type 3 (Type3) or Type 42 (TrueType)
#pdf.use14corefonts : False
#pdf.inheritcolor : False

### svg backend params
#svg.image_inline : True       ## write raster image data directly into the svg file
#svg.fonttype :   path         ## How to handle SVG fonts:
   ##     none: Assume fonts are installed on the machine where the SVG will be viewed.
   ##     path: Embed characters as paths -- supported by most SVG renderers
#svg.hashsalt : None           ## if not None, use this string as hash salt
                               ## instead of uuid4
### pgf parameter
#pgf.rcfonts : True
#pgf.preamble :            ## see text.latex.preamble for documentation
#pgf.texsystem : xelatex

### docstring params
##docstring.hardcopy = False  ## set this when you want to generate hardcopy docstring

## Event keys to interact with figures/plots via keyboard.
## Customize these settings according to your needs.
## Leave the field(s) empty if you don't need a key-map. (i.e., fullscreen : '')
#keymap.fullscreen : f, ctrl+f       ## toggling
#keymap.home : h, r, home            ## home or reset mnemonic
#keymap.back : left, c, backspace, MouseButton.BACK  ## forward / backward keys
#keymap.forward : right, v, MouseButton.FORWARD      ## for quick navigation
#keymap.pan : p                      ## pan mnemonic
#keymap.zoom : o                     ## zoom mnemonic
#keymap.save : s, ctrl+s             ## saving current figure
#keymap.help : f1                    ## display help about active tools
#keymap.quit : ctrl+w, cmd+w, q      ## close the current figure
#keymap.quit_all : W, cmd+W, Q       ## close all figures
#keymap.grid : g                     ## switching on/off major grids in current axes
#keymap.grid_minor : G               ## switching on/off minor grids in current axes
#keymap.yscale : l                   ## toggle scaling of y-axes ('log'/'linear')
#keymap.xscale : k, L                ## toggle scaling of x-axes ('log'/'linear')
#keymap.all_axes : a                 ## enable all axes
#keymap.copy : ctrl+c, cmd+c         ## Copy figure to clipboard

###ANIMATION settings
#animation.html :  none            ## How to display the animation as HTML in
                                   ## the IPython notebook. 'html5' uses
                                   ## HTML5 video tag; 'jshtml' creates a
                                   ## Javascript animation
#animation.writer : ffmpeg         ## MovieWriter 'backend' to use
#animation.codec : h264            ## Codec to use for writing movie
#animation.bitrate: -1             ## Controls size/quality tradeoff for movie.
                                   ## -1 implies let utility auto-determine
#animation.frame_format:  png      ## Controls frame format used by temp files
#animation.html_args:              ## Additional arguments to pass to html writer
#animation.ffmpeg_path:  ffmpeg    ## Path to ffmpeg binary. Without full path
                                   ## $PATH is searched
#animation.ffmpeg_args:            ## Additional arguments to pass to ffmpeg
#animation.avconv_path:  avconv    ## Path to avconv binary. Without full path
                                   ## $PATH is searched
#animation.avconv_args:            ## Additional arguments to pass to avconv
#animation.convert_path:  convert  ## Path to ImageMagick's convert binary.
                                   ## On Windows use the full path since convert
                                   ## is also the name of a system tool.
#animation.convert_args:           ## Additional arguments to pass to convert
#animation.embed_limit : 20.0      ## Limit, in MB, of size of base64 encoded
                                   ## animation in HTML (i.e. IPython notebook)

